Eulerian Motion Reconstruction for Water Scenery

Reconstructing and animating water scenery from nature produces compelling and immersive visual experiences. Previous work examined this task from the perspective of 2D video textures, with the goal of creating a looping video. In our work, we tackle the problem from a 3D perspective, creating a looping 4D dynamic reconstruction which can be interactively rendered from novel viewpoints from a single non-looping 2D source video. We represent motion as a 3D static \textit{Eulerian} motion field that advects canonical Gaussian splats that are cyclically reborn at fixed time periods, supervised using rendering losses. To model non-periodic and stochastic dynamics present in real-world scenes, we add a non-periodic, time-varying residual term to capture deviations from the static Eulerian motion field. We show quantitatively and qualitatively that our framework enables photorealistic animation of water scenes better than prior art.

==> tex_figures/alg1_propagation.tex <==
\begin{figure*}[t]
\centering
\begin{tikzpicture}[
  >=Latex, font=\small,
  gauss/.style={circle,draw=black,thick,minimum size=7pt,inner sep=0pt},
  edot/.style={circle,fill=black!45,minimum size=2.6pt,inner sep=0pt},
  canon/.style={star,star points=5,star point ratio=2.2,draw=black,
                minimum size=10pt,inner sep=0pt},
  lbl/.style={font=\scriptsize},
]

\begin{scope}[shift={(0,0)}]
  \def\tn{6}
  \def\L{9}

  \node[font=\bfseries,anchor=west] at (-0.3,4.3)
    {(a)~\textsc{PropForward}: $t_n$ Euler steps from $\mathbf{X}_n$};

  \coordinate (A0) at (0.2,3.0);
  \coordinate (A1) at (2.4,3.3);
  \coordinate (A2) at (4.6,1.9);
  \coordinate (A3) at (6.6,2.3);
  \draw[line width=3pt,gray!25] (A0) .. controls (A1) and (A2) .. (A3);

  \foreach \t in {0,...,\L}{
    \pgfmathsetmacro\s{\t/\L}
    \path (A0) .. controls (A1) and (A2) .. (A3) coordinate[pos=\s] (a\t);
  }
  \foreach \t in {1,...,\tn}{
    \pgfmathtruncatemacro\p{\t-1}
    \draw[-{Latex[length=2mm]},blue!70,thick] (a\p) -- (a\t);
  }
  \foreach \t in {0,...,\L}{ \node[edot] at (a\t) {}; }

  \node[canon,fill=orange!85] (ac) at (a0) {};
  \node[lbl,orange!70!black,above=2pt of ac,align=center]
    {canonical $\mathbf{X}_n$\\[-1pt]$t{=}0$};
  \node[gauss,fill=blue!75] (ag) at (a\tn) {};
  \node[lbl,blue!60!black,below=2pt of ag,align=center]
    {$\mathbf{X}_{n,i}$\\[-1pt]after $t_n$ steps};

  \node[lbl,text=black!60,above right=0pt and -6pt of a2]
    {$\mathbf{X}\!\gets\!\mathbf{X}+\mathbf{V}(\mathbf{X})$};
\end{scope}

\draw[gray!35] (7.5,-2.4) -- (7.5,4.2);

\begin{scope}[shift={(8.2,0)}]
  \def\L{15}
  \node[font=\bfseries,anchor=west] at (-0.3,4.3)
    {(b)~Random $T^{\mathrm{start}}_n$ stagger Gaussians over the cycle};

  \coordinate (B0) at (0.2,3.2);
  \coordinate (B1) at (3.0,3.4);
  \coordinate (B2) at (5.2,1.6);
  \coordinate (B3) at (8.4,1.4);
  \draw[line width=3pt,gray!25,-{Latex[length=3.5mm]}]
     (B0) .. controls (B1) and (B2) .. (B3);
  \node[gray!70] at (7.1,2.15) {$\mathbf{V}$};

  \foreach \t in {0,...,\L}{
    \pgfmathsetmacro\s{\t/\L}
    \path (B0) .. controls (B1) and (B2) .. (B3) coordinate[pos=\s] (b\t);
    \node[edot] at (b\t) {};
  }
  \node[canon,fill=orange!85] (bc) at (b0) {};
  \node[lbl,orange!70!black,below left=0pt and -6pt of bc]{rebirth $t{=}0$};

  \newcommand{\gb}[4]{
    \node[gauss,fill=#2!80] (bg#1) at (b#1) {};
    \node[lbl,text=#2!55!black,#4=1pt of bg#1,align=center]
      {$T^{\mathrm{start}}{=}#3$\\[-2pt]$t_n{=}#1$};}
  \gb{2}{green!60!black}{8}{above}
  \gb{6}{blue}{4}{above}
  \gb{9}{violet}{1}{below}
  \gb{12}{red}{13}{below}
\end{scope}

\node[draw,rounded corners,fill=black!3,align=left,inner sep=7pt,
      text width=15.6cm,font=\small] at (7.75,-1.55)
{
  \textbf{Algorithm~\ref{alg1} --- reconstruct frame $i$.}\;
  For each canonical Gaussian $n$:\hfill
  \textcolor{black!55}{\scriptsize e.g.\ $L{=}15,\,i{=}10$}\\[3pt]
  \makebox[0.8cm][l]{\footnotesize(3)} cycle index\quad
     $t_n \gets \bigl(i - T^{\mathrm{start}}_n\bigr)\bmod L$
     \hfill
     \textcolor{black!55}{\scriptsize $T^{\mathrm{start}}{=}4\!\Rightarrow\!t_n{=}6,\;\;
        T^{\mathrm{start}}{=}13\!\Rightarrow\!t_n{=}12$}\\[3pt]
  \makebox[0.8cm][l]{\footnotesize(4)} advect\quad
     $\mathbf{X}_{n,i} \gets \textsc{PropForward}(\mathbf{X}_n,\mathbf{V},t_n)$
     \quad\textcolor{black!55}{\scriptsize($t_n$ forward-Euler steps from the canonical position)}
};

\end{tikzpicture}
\caption{\textbf{Per-Gaussian random start-time forward propagation (Algorithm~\ref{alg1}).}
To reconstruct frame $i$, each canonical Gaussian is advected forward along the
Eulerian motion field $\mathbf{V}$ by its own cycle index
$t_n=(i-T^{\mathrm{start}}_n)\bmod L$.
\textbf{(a)}~\textsc{PropForward} takes $t_n$ forward-Euler steps
($\mathbf{X}\!\gets\!\mathbf{X}+\mathbf{V}(\mathbf{X})$) from the canonical position
$\mathbf{X}_n$ (the rebirth state at $t{=}0$).
\textbf{(b)}~Because each Gaussian is assigned a random start time
$T^{\mathrm{start}}_n\!\sim\!\mathrm{Uniform}[0,L]$, at any frame the Gaussians occupy
different cycle indices and are spread out along the ``conveyor belt,'' so their
rebirths are staggered across the loop rather than occurring all at once.}
\label{fig:alg1}
\end{figure*}


==> tex_figures/looping_sim.tex <==
\begin{figure*}[t]
\centering
\begin{tikzpicture}[
  >=Latex, font=\small,
  part/.style={circle,draw=black,thick,minimum size=9pt,inner sep=0pt},
]
\newcommand{\panel}[8]{
  \begin{scope}[xshift=#1 cm]
    \draw[rounded corners,gray!45,fill=gray!2] (0.05,-0.15) rectangle (2.95,6.05);
    \foreach \fx in {0.75,1.5,2.25}{
      \draw[gray!22,line width=2.4pt,-{Latex[length=2.4mm]}] (\fx,5.75) -- (\fx,0.15);}
    \newcommand\lane[4]{
      \node[circle,dashed,draw=##4!55,minimum size=9pt,inner sep=0pt] at (##1,##2){};
      \draw[##4!45,dotted,thick] (##1,##2) -- (##1,##3);
      \node[part,fill=##4!85] at (##1,##3){};}
    \lane{0.5}{5.0}{#4}{red}
    \lane{1.0}{5.3}{#5}{blue}
    \lane{1.5}{4.7}{#6}{green!60!black}
    \lane{2.0}{5.5}{#7}{violet}
    \lane{2.5}{5.0}{#8}{orange}
    \node[font=\bfseries] at (1.5,6.55) {#2};
    \node[font=\scriptsize\itshape,text=gray!60] at (1.5,6.28) {#3};
  \end{scope}}

\panel{0}{$i=0$}{}{5.0}{1.7}{2.0}{3.7}{4.1}
\panel{3}{$i=5$}{}{3.5}{4.7}{0.5}{2.2}{2.6}
\panel{6}{$i=10$}{}{2.0}{3.2}{3.5}{5.2}{1.1}
\panel{9}{$i=15$}{$\equiv i{=}0$}{5.0}{1.7}{2.0}{3.7}{4.1}
\panel{12}{$i=20$}{$\equiv i{=}5$}{3.5}{4.7}{0.5}{2.2}{2.6}
\panel{15}{$i=25$}{$\equiv i{=}10$}{2.0}{3.2}{3.5}{5.2}{1.1}

\draw[decorate,decoration={brace,amplitude=5pt},gray!70]
  (0.1,6.95) -- (8.9,6.95)
  node[midway,above=4pt,font=\small\bfseries,text=gray!70]{one cycle ($L=15$)};
\draw[decorate,decoration={brace,amplitude=5pt},teal!70]
  (9.1,6.95) -- (17.9,6.95)
  node[midway,above=4pt,font=\small\bfseries,text=teal!60!black]
  {repeats identically ($\equiv$ first cycle)};
\end{tikzpicture}
\caption{\textbf{Spatial looping simulation.}
Five Gaussians at different canonical positions (dashed rings), each assigned a
random start time $T^{\mathrm{start}}\!\sim\!\mathrm{Uniform}[0,L]$
(\textcolor{red!85}{$T{=}0$}, \textcolor{blue!85}{$T{=}3$},
\textcolor{green!55!black}{$T{=}6$}, \textcolor{violet}{$T{=}9$},
\textcolor{orange}{$T{=}12$}), are advected by a downward Eulerian motion field $\mathbf{V}$
with cycle length $L{=}15$. At frame $i$ each Gaussian sits
$t_n=(i-T^{\mathrm{start}})\bmod L$ forward-Euler steps below its canonical position
and snaps back on rebirth ($t_n{=}0$). Because the start times are staggered, the
Gaussians never reset all at once. The scene is exactly periodic:
frames $i{=}15,20,25$ reproduce $i{=}0,5,10$.}
\label{fig:looping_sim}
\end{figure*}


==> tex_figures/naive_looping.tex <==
\begin{figure*}[t]
\centering
\begin{tikzpicture}[
  >=Latex, font=\small,
  part/.style={circle,draw=black,thick,minimum size=9pt,inner sep=0pt},
]
\newcommand{\panel}[8]{
  \begin{scope}[xshift=#1 cm]
    \draw[rounded corners,gray!45,fill=gray!2] (0.05,-0.15) rectangle (2.95,6.05);
    \foreach \fx in {0.75,1.5,2.25}{
      \draw[gray!22,line width=2.4pt,-{Latex[length=2.4mm]}] (\fx,5.75) -- (\fx,0.15);}
    \pgfmathsetmacro\ylo{min(#4,#5,#6,#7,#8)}
    \pgfmathsetmacro\yhi{max(#4,#5,#6,#7,#8)}
    \fill[red!12,rounded corners] (0.18,\ylo-0.38) rectangle (2.82,\yhi+0.38);
    \draw[red!35,rounded corners,thick,dashed] (0.18,\ylo-0.38) rectangle (2.82,\yhi+0.38);
    \newcommand\lane[4]{
      \node[circle,dashed,draw=##4!55,minimum size=9pt,inner sep=0pt] at (##1,##2){};
      \draw[##4!45,dotted,thick] (##1,##2) -- (##1,##3);
      \node[part,fill=##4!85] at (##1,##3){};}
    \lane{0.5}{5.0}{#4}{red}
    \lane{1.0}{5.3}{#5}{blue}
    \lane{1.5}{4.7}{#6}{green!60!black}
    \lane{2.0}{5.5}{#7}{violet}
    \lane{2.5}{5.0}{#8}{orange}
    \node[font=\bfseries] at (1.5,6.55) {#2};
    \node[font=\scriptsize\itshape,text=gray!60] at (1.5,6.28) {#3};
  \end{scope}}

\panel{0}{$i=0$}{}{5.0}{5.3}{4.7}{5.5}{5.0}
\panel{3}{$i=5$}{}{3.5}{3.8}{3.2}{4.0}{3.5}
\panel{6}{$i=10$}{}{2.0}{2.3}{1.7}{2.5}{2.0}
\panel{9.8}{$i=15$}{$\equiv i{=}0$}{5.0}{5.3}{4.7}{5.5}{5.0}
\panel{12.8}{$i=20$}{$\equiv i{=}5$}{3.5}{3.8}{3.2}{4.0}{3.5}
\panel{15.8}{$i=25$}{$\equiv i{=}10$}{2.0}{2.3}{1.7}{2.5}{2.0}

\node[fill=red!80,text=white,font=\scriptsize\bfseries,rounded corners,inner sep=2pt]
  at (1.5,-0.55) {reset (all)};
\node[fill=red!80,text=white,font=\scriptsize\bfseries,rounded corners,inner sep=2pt]
  at (11.3,-0.55) {reset (all)};

\draw[-{Latex[length=3mm]},red!80,line width=1.4pt,
      decorate,decoration={snake,amplitude=1.1pt,segment length=6pt,post length=3mm}]
  (9.0,2.1) to[bend left=18] (9.75,5.0);
\node[red!80,font=\scriptsize\bfseries,align=center,rotate=64] at (9.15,3.7)
  {every Gaussian\\snaps back\\at once};

\draw[decorate,decoration={brace,amplitude=5pt},gray!70]
  (0.1,6.95) -- (8.9,6.95)
  node[midway,above=4pt,font=\small\bfseries,text=gray!70]{one cycle ($L=15$)};
\draw[decorate,decoration={brace,amplitude=5pt},red!70]
  (9.85,6.95) -- (18.75,6.95)
  node[midway,above=4pt,font=\small\bfseries,text=red!70!black]
  {repeats -- and jumps -- in lockstep};
\end{tikzpicture}
\caption{\textbf{Naive looping (shared start time) produces a jump artifact.}
If \emph{all} Gaussians share the same start time $T^{\mathrm{start}}{=}0$, then
$t_n = i \bmod L$ is identical for every particle: they advect as one rigid clump
(red band) and reset \emph{simultaneously} at $i=0,15,\dots$, so the entire scene
teleports back to the canonical positions in a single frame. Compare to our
staggered scheme (Fig.~\ref{fig:looping_sim}), where random start times spread the
resets across the cycle.}
\label{fig:naive_looping}
\end{figure*}


==> tex_figures/pipeline_tikz.tex <==
\begin{figure*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tikzpicture}[
  >=Latex, font=\small,
  stage/.style={rounded corners=3pt,draw=#1!60,fill=#1!12,thick},
  titl/.style={font=\bfseries\small,anchor=north west},
  lbl/.style={font=\scriptsize,align=center},
  lane/.style={font=\scriptsize,anchor=north west,align=left},
  flow/.style={-{Latex[length=2.6mm]},line width=1.1pt,black!70},
  sflow/.style={-{Latex[length=1.8mm]},line width=0.8pt,black!55},
  bflow/.style={-{Latex[length=2.6mm]},line width=1.1pt,red!75,dashed},
  rin/.style={rounded corners=2pt,draw=blue!45,fill=white,font=\scriptsize,
              align=center,inner sep=2pt,minimum width=1.3cm,minimum height=0.42cm},
  rmlp/.style={rounded corners=2pt,draw=blue!60,fill=blue!18,thick,font=\scriptsize,align=center},
  rout/.style={rounded corners=2pt,draw=blue!45,fill=white,font=\scriptsize,align=center,inner sep=3pt},
  splat/.style={ellipse,draw=black!70,inner sep=0pt,minimum width=10pt,minimum height=5pt},
  msplat/.style={ellipse,draw=black!60,inner sep=0pt,minimum width=6pt,minimum height=3pt},
]

\newcommand{\framestack}[2]{
  \draw[fill=white,draw=black!50] (#1+0.16,#2+0.16) rectangle +(1.35,0.95);
  \draw[fill=white,draw=black!50] (#1+0.08,#2+0.08) rectangle +(1.35,0.95);
  \draw[fill=blue!6,draw=black!70] (#1,#2) rectangle +(1.35,0.95);
  \draw[blue!60!cyan,line width=0.8pt,decorate,decoration={snake,amplitude=1pt,segment length=5pt}]
    (#1+0.15,#2+0.32) -- +(1.05,0);
  \draw[blue!40!cyan,line width=0.8pt,decorate,decoration={snake,amplitude=1pt,segment length=5pt}]
    (#1+0.15,#2+0.58) -- +(1.05,0);}

\newcommand{\cluster}[2]{
  \node[splat,fill=red!75,rotate=20]    at (#1-0.30,#2+0.10) {};
  \node[splat,fill=blue!75,rotate=-15]  at (#1+0.28,#2+0.22) {};
  \node[splat,fill=green!60!black,rotate=45,opacity=0.9] at (#1+0.02,#2-0.20) {};
  \node[splat,fill=orange!90,rotate=-40] at (#1+0.42,#2-0.18) {};
  \node[splat,fill=violet!80,rotate=5]  at (#1-0.38,#2-0.32) {};}

\newcommand{\advpanel}[5]{
  \draw[dashed,fill=gray!12,draw=black!55]
    (#1,#2+#5) -- (#1+0.30,#2+#5+0.22) -- (#1+#4+0.30,#2+#5+0.22) -- (#1+#4,#2+#5) -- cycle;
  \draw[dashed,fill=gray!22,draw=black!55]
    (#1+#4,#2) -- (#1+#4+0.30,#2+0.22) -- (#1+#4+0.30,#2+#5+0.22) -- (#1+#4,#2+#5) -- cycle;
  \draw[dashed,fill=white,draw=black!55] (#1,#2) rectangle +(#4,#5);
  \foreach \u/\amp/\seg in {0.165/1.0pt/9pt, 0.359/0.7pt/12pt, 0.524/1.2pt/8pt,
                            0.688/0.8pt/13pt, 0.853/1.05pt/10.5pt}{
    \pgfmathsetmacro\fx{#1+\u*#4}
    \draw[gray!45,line width=1.1pt,-{Latex[length=1.8mm]},decorate,
          decoration={snake,amplitude=\amp,segment length=\seg,post length=2.2mm}]
      (\fx,#2+0.93*#5) -- (\fx,#2+0.07*#5);}
  \foreach \u/\off/\dy/\c/\rot in {0.200/0/0.05/red!75/20, 0.329/3/-0.06/blue!75/-15,
                                   0.565/1/0.07/green!60!black/45, 0.665/4/-0.03/orange!90/-40,
                                   0.871/2/0.06/violet!80/5}{
    \pgfmathsetmacro\sx{#1+\u*#4}
    \pgfmathsetmacro\sy{#2+#5*(1.38-0.30*mod(#3+\off,5)+\dy)/1.75}
    \node[msplat,fill=\c,rotate=\rot] at (\sx,\sy) {};}}

\draw[stage=orange] (0,5.40) rectangle (5.45,8.35);
\node[titl] at (0.08,8.30) {Stage 1: Static Reconstruction};
\framestack{0.35}{6.20}
\node[lbl] at (1.05,5.90) {input video $\{I_i\}_{i=1}^{F}$};
\draw[flow] (2.05,6.70) -- (2.75,6.70) node[midway,above,lbl] {3DGS};
\cluster{3.85}{6.95}
\node[lbl] at (3.95,5.85) {canonical Gaussians\\[-2pt]$\{{\bf G}_n\}_{n=1}^{N}$};

\draw[stage=green] (0,0.45) rectangle (5.45,3.75);
\node[titl] at (0.08,3.70) {Stage 2: Motion Field Pretraining};
\draw[fill=white,draw=black!60] (0.35,1.55) rectangle +(1.35,0.95);
\foreach \p/\q/\c in {0.55/1.75/cyan,0.95/2.15/magenta,1.25/1.85/yellow!70!orange,0.75/2.0/teal}{
  \draw[\c!80!black,-{Latex[length=1.2mm]},line width=0.8pt] (\p,\q) -- +(0.22,-0.13);}
\node[lbl] at (1.05,1.25) {2D optical flow};
\draw[flow,black!50] (5.1,5.40) -- (5.1,3.4) node[pos=0.22,left,lbl,black!60] {depth, poses};
\draw[flow] (1.85,2.05) -- (2.55,2.05) node[midway,above,lbl] {lift\\[-3pt]to 3D};
\draw[fill=gray!12,draw=black!60]
  (2.75,2.75) -- (3.03,2.95) -- (4.63,2.95) -- (4.35,2.75) -- cycle;
\draw[fill=gray!22,draw=black!60]
  (4.35,1.35) -- (4.63,1.55) -- (4.63,2.95) -- (4.35,2.75) -- cycle;
\draw[fill=white,draw=black!60] (2.75,1.35) rectangle +(1.6,1.4);
\foreach \fx in {3.05,3.55,4.05}{
  \draw[gray!45,line width=1.8pt,-{Latex[length=1.8mm]}] (\fx,2.6) -- (\fx,1.5);}
\foreach \fx in {3.25,3.75,4.25}{
  \draw[gray!30,line width=1.2pt,-{Latex[length=1.2mm]}] (\fx+0.12,2.9) -- (\fx+0.02,2.79);}
\node[lbl] at (3.55,1.05) {3D Eulerian motion\\[-2pt]field ${\bf V}({\bf X})$};

\draw[stage=yellow] (5.95,0.45) rectangle (19.00,8.35);
\node[titl] at (6.03,8.30) {Stage 3: Looping Dynamic Reconstruction};

\draw[rounded corners=2pt,fill=white,draw=black!35] (13.05,7.18) rectangle (18.90,8.32);
\node[anchor=north west,align=left,font=\scriptsize] at (13.18,8.30)
 {\textbf{per-Gaussian schedule} (random $T^{\mathrm{start}}_n$)\\
  cycle index\ \ $t_n=(i-T^{\mathrm{start}}_n)\bmod L$\\
  cycle number\ $p_n=\big\lfloor (i-T^{\mathrm{start}}_n)/L\big\rfloor$};

\draw[rounded corners=2pt,fill=white,draw=black!30] (6.45,4.30) rectangle (11.20,7.05);
\node[font=\scriptsize,anchor=west,fill=white,inner sep=2pt] at (6.70,7.05)
  {\textbf{Training (Alg.\,1)} -- random frame $i$};
\cluster{6.95}{5.85}
\foreach \sy/\sx/\lab/\c in {6.25/7.80/1/red!80!black, 6.02/8.45/2/blue!80!black,
                             5.79/8.00/3/green!55!black, 5.56/8.30/4/orange!95!black,
                             5.33/8.10/5/violet!85!black}{
  \draw[sflow] (\sx,\sy) -- (9.50,\sy);
  \node[font=\tiny,anchor=east,inner sep=1.5pt,text=\c] at (\sx,\sy) {$t_\lab$};}
\advpanel{9.55}{5.30}{3}{1.10}{1.10}
\node[lbl,font=\tiny] at (10.10,6.78) {frame $i$};
\node[lbl,font=\tiny] at (7.70,4.95) {different $t_n$ per Gaussian;\\[-2pt]no state kept};
\node[circle,draw=black!65,fill=white,inner sep=1pt,font=\small] (addT) at (10.10,4.62) {$\oplus$};
\draw[flow] (10.10,5.30) -- (addT.north);

\draw[rounded corners=2pt,fill=white,draw=black!30] (11.45,4.30) rectangle (18.90,7.05);
\node[font=\scriptsize,anchor=west,fill=white,inner sep=2pt] at (11.70,7.05)
  {\textbf{Inference (Alg.\,2)} -- one Euler step per frame};
\advpanel{12.10}{5.30}{0}{1.10}{1.10}
\advpanel{13.95}{5.30}{1}{1.10}{1.10}
\advpanel{15.80}{5.30}{2}{1.10}{1.10}
\node[lbl,font=\tiny] at (12.65,6.78) {frame 1};
\node[lbl,font=\tiny] at (14.50,6.78) {frame 2};
\node[lbl,font=\tiny] at (16.35,6.78) {frame $L$};
\draw[flow] (13.54,5.85) -- (13.91,5.85) node[midway,above=-1pt,lbl,font=\tiny] {$+1$};
\draw[flow] (15.39,5.85) -- (15.76,5.85) node[midway,above=-1pt,lbl,font=\tiny] {$\cdots$};
\draw[flow] (16.35,5.30) .. controls (15.5,4.62) and (13.2,4.62) .. (12.65,5.30);
\node[lbl,font=\tiny,fill=white,inner sep=1pt] at (14.50,4.86) {reborn at $t_n{=}0$};
\node[circle,draw=black!65,fill=white,inner sep=1pt,font=\small] (addI) at (17.75,5.85) {$\oplus$};
\draw[flow] (17.24,5.85) -- (addI.west);
\draw[flow] (addI.south) -- (17.75,4.55) -- (17.15,4.55);
\node[align=center,font=\scriptsize\bfseries,text=teal!50!black] at (14.85,4.55)
 {$\Rightarrow$ infinitely-looping 4D scene\\[-2pt] rendered from novel views};
\draw[flow] (10.99,5.85) -- (12.10,5.85)
  node[midway,above=-2pt,lbl,font=\tiny,fill=white,inner sep=1pt] {one jump};

\draw[rounded corners=2pt,fill=blue!7,draw=blue!40] (9.20,2.35) rectangle (15.60,4.05);
\node[font=\scriptsize\bfseries,anchor=west,fill=blue!7,inner sep=2pt,text=blue!45!black]
  at (9.45,4.05) {shared non-periodic residual field ${\bf D}$};
\node[rin] (rX) at (10.30,3.58) {${\bf X}$\\[-3pt]\tiny canonical pos.};
\node[rin] (rt) at (10.30,3.06) {$t_n$\\[-3pt]\tiny cycle index};
\node[rin] (rp) at (10.30,2.58) {$p_n$\\[-3pt]\tiny cycle number};
\node[rmlp,minimum width=1.1cm,minimum height=1.1cm] (rD) at (12.30,3.06)
  {${\bf D}$\\[-2pt]\tiny MLP};
\draw[sflow] (rX.east) -- (rD.west);
\draw[sflow] (rt.east) -- (rD.west);
\draw[sflow] (rp.east) -- (rD.west);
\node[rout] (rO) at (14.20,3.06) {$\Delta{\bf X},\,\Delta{\bf C},\,\Delta\mathrm{O}$};
\draw[sflow] (rD.east) -- (rO.west);
\node[lbl,font=\tiny,text=blue!45!black] at (14.20,2.56) {at inference: $p_n{=}0$};
\draw[sflow] (14.20,3.30) -- (14.20,4.22) -- (10.70,4.22) -- (10.70,4.62) -- (addT.east);
\draw[sflow] (14.20,4.22) -- (18.45,4.22) -- (18.45,5.85) -- (addI.east);
\fill[black!55] (14.20,4.22) circle (0.045);

\draw[flow] (addT.west) -- (8.80,4.62) -- (8.80,2.05);
\node[lbl,fill=white,inner sep=1pt] at (8.80,3.35) {rasterize};
\draw[fill=white,draw=black!70] (8.15,1.0) rectangle +(1.5,1.05);
\draw[blue!60!cyan,line width=0.8pt,decorate,decoration={snake,amplitude=1pt,segment length=5pt}]
  (8.3,1.35) -- +(1.2,0);
\draw[blue!40!cyan,line width=0.8pt,decorate,decoration={snake,amplitude=1pt,segment length=5pt}]
  (8.3,1.66) -- +(1.2,0);
\node[lbl] at (8.9,0.72) {rendered $\hat{I}_i$};
\framestack{11.3}{1.03}
\node[lbl] at (12.0,0.72) {input frame $I_i$};
\draw[{Latex[length=2mm]}-{Latex[length=2mm]},line width=1pt,black!70] (9.75,1.5) -- (11.2,1.5)
  node[midway,above,lbl] {$\mathcal{L}_1$ + SSIM};

\draw[bflow] (10.5,1.15) .. controls (12.8,0.6) and (14.6,0.9) .. (15.60,2.30);
\node[align=left,font=\scriptsize,text=red!70!black,anchor=west] at (15.45,2.60)
 {backpropagate: jointly\\ optimize $\{{\bf G}_n\}$, ${\bf V}$, and ${\bf D}$};

\draw[flow] (5.45,6.30) -- (6.45,6.30) node[pos=0.30,above,lbl] {$\{{\bf G}_n\}$};
\draw[flow] (5.45,2.05) -- (6.20,2.05) -- (6.20,5.30) -- (6.45,5.30);
\node[lbl,anchor=west] at (5.5,1.75) {${\bf V}$};
\fill[yellow!12] (6.11,4.01) rectangle (6.29,4.19);
\fill[yellow!12] (8.71,4.01) rectangle (8.89,4.19);
\draw[sflow] (5.80,6.30) -- (5.80,4.10) -- (10.30,4.10) -- (10.30,3.82);
\fill[black!70] (5.80,6.30) circle (0.05);

\end{tikzpicture}
}
\caption{\textbf{Method overview.}
\textbf{(Stage 1)} A static 3DGS reconstruction of the input monocular video
(ignoring motion) initializes the canonical Gaussians $\{{\bf G}_n\}$.
\textbf{(Stage 2)} 2D optical flow between adjacent frames is lifted to 3D using
depth and camera poses from Stage~1; the resulting (position, scene flow) pairs
pretrain the static Eulerian motion field ${\bf V}({\bf X})$.
\textbf{(Stage 3)} Every Gaussian carries its own random start time
$T^{\mathrm{start}}_n$, hence its own cycle index $t_n$ and cycle number $p_n$
(top-right box).
\emph{Training} (left panel, Alg.~\ref{alg1}): a random frame $i$ is reconstructed by
jumping each Gaussian directly from its canonical state by $t_n$ forward-Euler steps of
${\bf V}$ -- the arrow lengths differ because the $t_n$ do -- so no state is carried
between frames.
\emph{Inference} (right panel, Alg.~\ref{alg2}): that same jump is run once to obtain
frame~1, after which every Gaussian advances a single Euler step per frame and returns
to its canonical state when $t_n{=}0$; the staggered start times spread these rebirths
over the whole cycle.
Both modules share the same non-periodic residual field ${\bf D}$ (centre block),
which takes the canonical position
${\bf X}$, the cycle index $t_n$, and the cycle number $p_n$, and predicts offsets
$\Delta{\bf X},\Delta{\bf C},\Delta\mathrm{O}$ that are added to the propagated
Gaussians; at inference ${\bf D}$ is queried with the first cycle only ($p_n{=}0$)
so that the residuals repeat as well.
The resulting Gaussians are rasterized and compared against the input frame with
$\mathcal{L}_1$ and SSIM losses, jointly optimizing $\{{\bf G}_n\}$, ${\bf V}$, and
${\bf D}$, yielding an infinitely-looping 4D scene.}
\label{fig:pipeline_tikz}
\end{figure*}

